Energy and Momentum Distribution of Surface Plasmon-induced Hot Carriers Isolated via Spatiotemporal Separation

Understanding the differences between photon-induced and plasmon-induced hot electrons is essential for the construction of devices for plasmonic energy conversion. The mechanism of the plasmonic enhancement in photochemistry, photocatalysis, and light-harvesting and especially the role of hot carriers is still heavily discussed. The question remains, if plasmon-induced and photon-induced hot carriers are fundamentally different, or if plasmonic enhancement is only an effect of field concentration producing these carriers in greater numbers. For the bulk plasmon resonance, a fundamental difference is known, yet for the technologically important surface plasmons this is far from being settled. The direct imaging of surface plasmon-induced hot carriers could provide essential insight, but the separation of the influence of driving laser, field-enhancement, and fundamental plasmon decay has proven to be difficult. Here, we present an approach using a two-color femtosecond pump-probe scheme in time-resolved 2-photon-photoemission (tr-2PPE), supported by a theoretical analysis of the light and plasmon energy flow. We separate the energy and momentum distribution of the plasmon-induced hot electrons from the one of photoexcited electrons by following the spatial evolution of photoemitted electrons with energy-resolved Photoemission Electron Microscopy (PEEM) and Momentum Microscopy during the propagation of a Surface Plasmon Polariton (SPP) pulse along a gold surface. With this scheme, we realize a direct experimental access to plasmon-induced hot electrons. We find a plasmonic enhancement towards high excitation energies and small in-plane momenta, which suggests a fundamentally different mechanism of hot electron generation, as previously unknown for surface plasmons.

==> arxiv upload/authors.tex <==
% \newcommand{\titlestr}{Spatiotemporal Separation of Plasmon-induced Hot Carriers in Time- and Energy-resolved Photoemission Electron Microscopy}
%\newcommand{\titlestr}{Spatiotemporal Separation and Momentum Distribution of Plasmon-induced Hot Carriers}
\newcommand{\titlestr}{Energy and Momentum Distribution of Surface Plasmon-induced Hot Carriers Isolated via Spatiotemporal Separation}

\author{Michael Hartelt} % 0000-0002-0356-6662
\email{hartelt@physik.uni-kl.de}

\author{Pavel N. Terekhin} % 0000-0002-6616-7351
\author{Tobias Eul} % 0000-0002-7362-6448
\author{Anna-Katharina Mahro} % 0000-0001-5856-0367
\author{Benjamin Frisch}
\author{Eva Prinz} % 0000-0002-9880-5186
\affiliation{Department of Physics and Research Center OPTIMAS, TU Kaiserslautern, Germany}

%\author{Mirko Cinchetti}
%\affiliation{Experimentelle Physik VI, Fakult\"at Physik, TU Dortmund, Germany}

\author{Baerbel Rethfeld}
\affiliation{Department of Physics and Research Center OPTIMAS, TU Kaiserslautern, Germany}	

\author{Benjamin Stadtm\"uller} % 0000-0001-8439-434X
\affiliation{Department of Physics and Research Center OPTIMAS, TU Kaiserslautern, Germany}	
%\affiliation{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Mainz 55128, Germany}	

\author{Martin Aeschlimann} % 0000-0003-3413-5029
\affiliation{Department of Physics and Research Center OPTIMAS, TU Kaiserslautern, Germany}	
